DiscoPrompt: Path Prediction Prompt Tuning for Implicit Discourse Relation Recognition

Implicit Discourse Relation Recognition (IDRR) is a sophisticated and challenging task to recognize the discourse relations between the arguments with the absence of discourse connectives. The sense labels for each discourse relation follow a hierarchical classification scheme in the annotation process (Prasad et al., 2008), forming a hierarchy structure. Most existing works do not well incorporate the hierarchy structure but focus on the syntax features and the prior knowledge of connectives in the manner of pure text classification. We argue that it is more effective to predict the paths inside the hierarchical tree (e.g., "Comparison -> Contrast -> however") rather than flat labels (e.g., Contrast) or connectives (e.g., however). We propose a prompt-based path prediction method to utilize the interactive information and intrinsic senses among the hierarchy in IDRR. This is the first work that injects such structure information into pre-trained language models via prompt tuning, and the performance of our solution shows significant and consistent improvement against competitive baselines.

==> sections/experiments_result.tex <==
\begin{table*}[!ht]
\centering
\vspace{-0.5cm}
\small
  \scalebox{0.9}{\begin{tabular}{l| cc | cc | cc | cc }
    \toprule
    % \multirow{2}{*}{Data} &
    %   \multirow{2}{*}{ Models } &
    \multirow{2}{*}{\textbf{Models} } &    
    % \multicolumn{2}{c|}{\textbf{PDTB 2.0-Ji (Top)}} &
    % \multicolumn{2}{c|}{\textbf{PDTB 2.0-Ji (Second)}} &
    % \multicolumn{2}{c|}{\textbf{PDTB 2.0-Lin (Top)}} &
    % \multicolumn{2}{c}{\textbf{PDTB 2.0-Lin (Second)}} \\
    \multicolumn{2}{c|}{\textbf{Ji (Top)}} &
    \multicolumn{2}{c|}{\textbf{Ji (Second)}} &
    \multicolumn{2}{c|}{\textbf{Lin (Top)}} &
    \multicolumn{2}{c}{\textbf{Lin (Second)}} \\
    { } & {\textbf{F1}} & {\textbf{Accuracy}} & {\textbf{F1}}& {\textbf{Accuracy}} & {\textbf{F1}} & {\textbf{Accuracy}} & {\textbf{F1}} & {\textbf{Accuracy}} \\
    \midrule
    % DISCO2~\cite{DBLP:journals/tacl/JiE15} & - & - & -  & 44.59 & - & - & - & - \\  
    % DER~\cite{Bai2018Deep}  & 51.06 & - & - & 48.22  & - & - & - & 45.73 \\
    MTL-MLoss~\cite{DBLP:conf/acl/NguyenLTN19}  & 53.00 & - & - & 49.95& - & - & - & 46.48\\
    ELMo-C\&E~\cite{Dai2019A}  & 52.89 & 59.66 & 33.41 & 48.23  & - & - & - & -\\
    RWP-CNN\cite{DBLP:conf/sigdial/VariaHC19} & 50.20 & 59.13 & - & - & - & - & - & -\\ 
    TransS\cite{DBLP:conf/acl/HeWGH20}  & - & - & - & - & 51.24 & 59.94 & - & -\\ 
    BMGF-RoBERTa~\cite{DBLP:conf/ijcai/LiuOSJ20}^* & 63.39 & 69.06 & 35.25 & 58.13 & 58.54 & 68.66 & 39.15 & 53.96 \\    
    % CG-T5~\cite{DBLP:conf/emnlp/JiangFCLZ21}  & 57.18 & - & 37.76 & - & - & - & - & -\\
    LDSGM~\cite{DBLP:conf/aaai/WuCGLZS22}  & 63.73 &  71.18 & 40.49 & 60.33 & - & - & - & - \\
    ContrastiveIDRR\footnotemark[2]~\cite{conf/emnlp/Contrastive_Learning} & \underline{67.85} &  71.70 & \underline{45.54} & 59.19 & - & - & - & - \\
    % ContrastiveIDRR (w data augmentation)~\cite{conf/emnlp/Contrastive_Learning} & 69.60 &  72.18 & 49.66 & 61.69 & - & - & - & - \\    
    % ContrastiveIDRR (w/o data augmentation) & \underline{67.85} &  71.70 & \underline{45.54} & 59.19 & - & - & - & - \\
    % ContrastiveIDRR (w data augmentation) & 69.60 &  72.18 & 49.66 & 61.69 & - & - & - & - \\    
    
    \midrule
    % RoBERTa-base~\cite{DBLP:journals/corr/abs-1907-11692} & 60.29 & 68.93 & 39.43 & 58.90 & 56.33 & 70.61 & 38.11 & 57.83\\ 
    % RoBERTa-large~\cite{DBLP:journals/corr/abs-1907-11692} & 67.38 & 74.76 & 38.67 & 60.64 & 57.83 & 73.47 & 41.76 & 60.57\\
    XLNet (base, cased)~\cite{DBLP:conf/acl/KimFGL20}^*  & 59.33 & 66.35 & 36.36 & 54.73 & 56.16 & 68.05 & 36.23 & 55.82\\
    XLNet (large, cased)~\cite{DBLP:conf/acl/KimFGL20}^*   & 63.58 & 69.52 & 38.24 & 61.29 & 58.97 & \underline{72.17} & 40.71 & 58.77\\
    OTMT (XLNet-base)~\cite{DBLP:conf/www/JiangQL22}  &  60.78 & 68.89 & - & 56.65 & - & - & - & 56.37\\
    OTMT (XLNet-large)~\cite{DBLP:conf/www/JiangQL22}  & 64.46 & 72.34 & - & 61.06 & - & - & - & \underline{61.62}\\
    %\midrule  
    T5-base (\jy{Fine-Tuning})~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}^* & 57.61 & 65.39 & 33.96 & 55.53 & 50.50 & 63.59 & 36.49 & 51.96\\
    T5-large (\jy{Fine-Tuning})~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}^* & 61.37 & 69.69 & 38.04 & 57.65 & 58.12 & 71.13 & 42.04 & 59.40\\
    % T5-large (fine-tune)~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} & 61.37 & 69.69 & 38.04 & 57.65 & \underline{61.98} & \underline{72.17} & \underline{43.63} & 59.66\\
    \midrule
    Prefix-Tuning (T5-base)~\cite{DBLP:conf/acl/LiL20}^* & 25.87 & 52.45 & 7.49  & 31.09  & 25.08 & 54.18 & 8.45 & 26.37\\
    Prefix-Tuning (T5-large)~\cite{DBLP:conf/acl/LiL20}^* & 63.74 & 71.51 & 39.73 & 59.77 & 58.06 & 69.84 & 36.86 & 56.53\\
    Prompt-Tuning (T5-base)~\cite{DBLP:conf/emnlp/LesterAC21}^* & 30.17 & 56.11 & 15.01 & 38.21 & 25.26 & 55.09 & 8.97 & 27.68\\
    Prompt-Tuning (T5-large)~\cite{DBLP:conf/emnlp/LesterAC21}^* & 66.95 & 71.99 & 44.08 & 60.15 &  \underline{59.92} &  71.02 & 40.75 & 60.44\\
    % PCP w/ RoBERTa-base~\cite{DBLP:journals/corr/abs-2210-07032} & 64.95 & 70.84 & 41.55 & 60.54  & - & -  & - & -\\     
    PCP (RoBERTa-base)~\cite{DBLP:journals/corr/abs-2210-07032}^* & 64.95 & 70.84 & 41.55 & 60.54 & 53.00 & 66.58 & 41.19 & 56.14 \\     
    % PCP w/ RoBERTa-large~\cite{DBLP:journals/corr/abs-2210-07032} & 67.79 & \underline{73.80} & 44.04 & \underline{61.41}  & - & -  & - & -\\    
    PCP (RoBERTa-large)~\cite{DBLP:journals/corr/abs-2210-07032}^* & 67.79 & \underline{73.80} & 44.04 & \underline{61.41}  & 52.75 & 71.13  & \underline{43.04} & 60.44 \\    
    \midrule    
    % \bf DiscoPrompt (T5-base) & 63.84 & 69.01 & 43.32 & 59.19  & 62.56 & 68.54  & 37.67 & 55.09\\
    % \bf DiscoPrompt (T5-base) & 64.29 & 70.55 & 43.38 & 60.15  & 58.16 & 67.75  & 35.81 & 56.14\\ %Lin setting
    % DiscoPrompt (T5-base) & 64.29 & 70.55 & 43.38 & 60.15  & 62.56 & 68.54  & 37.67 & 55.09\\ %Lin setting
    DiscoPrompt (T5-base) & 65.79 & 71.70 & 43.68 & 61.02  & 64.90 & 71.28  & 41.82 & 59.27\\ 
    % \midrule
    % DiscoPrompt (T5-large) & 68.19 & 73.82 &  45.85 &  63.43 &  66.18 & 73.76 &  45.77 & 64.10\\ % Run 5 times and determinter which one (learning rate 0.06)
    % DiscoPrompt (T5-v1\_1-large) & 69.83 & 74.11 & 44.26 & 64.20 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-large)(relation path) & 69.70 & 74.01 & \bf49.61 & 64.10 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-large)(relation path;) & \bf72.08 & 75.46 & 44.67 & \bf65.16 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-large)(path is) & 70.28 & 74.40 & 45.94 & 64.97 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-large) & \bf70.84 & \bf75.65 & \bf49.03 & \bf64.58 & \bf69.17 & \bf74.80 & \bf46.35 & \bf62.27\\
    DiscoPrompt (T5-large) & \bf70.84 & \bf75.65 & \bf49.03 & \bf64.58 & \bf67.06 & \bf73.76 & \bf45.25 & \bf63.05\\
    % DiscoPrompt (T5-v1\_1-large)(path is.) & 70.39 & 74.40 & 44.76 & 65.06 & - & - & - & -\\
    % \midrule
    % \bf DiscoPrompt (T5-base) & 63.84 & 69.01 & 43.32 & 59.19  & 62.56 & 68.54  & 37.67 & 55.09\\
    % \bf DiscoPrompt (T5-base) & 64.29 & 70.55 & 43.38 & 60.15  & 58.16 & 67.75  & 35.81 & 56.14\\ %Lin setting
    % DiscoPrompt (T5-base) & 64.29 & 70.55 & 43.38 & 60.15  & 62.56 & 68.54  & 37.67 & 55.09\\ %Lin setting
    % DiscoPrompt (t5-v1\_1-base)(path is;) & 65.79 & 71.70 & 43.68 & 61.02  & - & - & - & -\\
    % \bf DiscoPrompt (T5-large) & \bf66.53 & \bf 73.15 & \bf 46.12 & \bf 63.81 & \bf 66.18 & \bf 73.76 & \bf 45.77 & \bf 64.10\\ % Run 5 times and determinter which one (learning rate 0.05)
    % DiscoPrompt (T5-3B)  & 70.48 & 76.23 & 48.29 & 65.74 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-xl)(path is; bs16) & 70.53 & 75.75 & 50.29 & 65.35  & - & - & - & -\\   
    % DiscoPrompt (T5-v1\_1-xl)(bs16) & 69.94 & 76.03 & 48.30 & 66.12  & - & - & - & -\\
    % \midrule
    % DiscoPrompt (T5-11B) & 71.84 & 76.80 & 47.74 & 65.83 & - & - & - & -\\ 
    % DiscoPrompt (T5-11B) & 72.38 & 77.19 & 43.12 & 68.05 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-xxl) & 74.14 & 78.44 & 51.66 & 67.76 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-xxl) & \bf75.83 & 78.73 & 51.15 & \bf68.82 & - & - & - & -\\
    % DiscoPrompt (T5-v1\_1-xxl) & 74.45 & \bf79.11 & \bf53.16 & 68.72 & - & - & - & -\\
    \midrule    
    % DiscoPrompt (t5-v1\_1-xl) & 73.53 & 77.86 & 44.39 & 66.51 & 69.69  & 77.02 & 45.88 & 64.75\\
    DiscoPrompt (T5-11b) & 75.34 & 78.06 & 52.42 & 68.14  & 72.78 & 77.55 & 47.18 & 67.62\\ 
    \bottomrule
  \end{tabular}}
  \vspace{-0.05in}
  \caption{
  \label{tab:discourse relation classification PDTB 2.0}
The accuracy (\%) and F1 score (\%) are evaluated on the PDTB 2.0 dataset. * marks the results of reproduced models. More baselines before 2019 can be found in Table~\ref{tab:Appendix_discourserelation_classification_pdtb2.0} in Appendix.
}
\vspace{-0.5cm}
\end{table*}
% \footnotetext[6]{We use the average results of their best single model.}


\section{Experimental Result}
\footnotetext[2]{We use their model without a data augmentation version for a fair comparison. This model with data augmentation version is also appended in Table~\ref{tab:Appendix_discourserelation_classification_pdtb2.0} in Appendix.}

\subsection{Main Results}
Table~\ref{tab:discourse relation classification PDTB 2.0} and Table~\ref{tab:discourserelation classification CoNLL16} summarize the main results of the PDTB 2.0 and CoNLL-2016 \xin{datasets}, from which we derive the following conclusions.
\textbf{First}, our method significantly outperforms all baselines and achieves state-of-the-art performance at both top and second-level classes in the IDRR task.
Specifically, our method gains a considerable improvement of 6.93\% second-level accuracy, 10.99\% second-level F1 score, 5.96\% top-level accuracy, and 9.47\% top-level F1 score over the fine-tuning of the T5-large model in \xin{PDTB 2.0 (\textit{Ji})}.
It demonstrates that our method effectively \xin{utilizes} the structure information and \xin{perceives the} specific knowledge on the correlation of discourse relations and connectives 
% for enhancing the ability of the T5 model to undertake this task.
\xin{and finally enhances the ability of T5 to undertake this challenging task.}
\textbf{Second}, the prompt-based baselines \xin{(e.g., Prefix-Tuning, PromptTuning, and PCP)} receive outstanding performance and perform better than the T5-large \jy{fine-tuning} method on this task.
% It may attribute to prompt-based methods efficiently utilizing the limited training instances of the specific second-level classes (e.g., \textit{Temp.Synchrony}) by updating a few learnable parameters, as shown in many previous works~\cite{DBLP:conf/naacl/ScaoR21,DBLP:conf/emnlp/LesterAC21}, whereas the T5-large model tends to overfit these considerably fewer training data by fine-tuning all learnable parameters of the model.
\xin{Many works~\cite{DBLP:conf/naacl/ScaoR21,DBLP:conf/emnlp/LesterAC21} has discussed the overfitting problem of T5-large fine-tuning, and this can be partially solved by prompt-tuning by updating a few learnable parameters with limited training instances.}
The learnable parameters of baselines and \xin{DiscoPrompt} are shown in Appendix~\ref{sec:appendix_approximation_learnable parameters}.  
% \textbf{Third}, the ContrastiveIDRR and our method obtain better performance on the F1 score evaluation metric. 
\textbf{Third}, the ContrastiveIDRR and our method obtain better F1 scores.
% It may result from our path prediction method integrating the dependencies between the top-level relations, second-level types, and the decided connectives in the labels hierarchy.
\xin{This observation can support the necessity of integrating the dependencies among relations as well as connectives in the label hierarchy.}



% \noindent \textbf{T5-11B Performance}
Fine-tuning a relatively \jy{pre-trained} large language model (LLM) such as T5-11b \xin{requires} extensive computation \jy{resources} to update all trainable parameters.
% of the whole \jy{pre-trained} language model (PLM).
However, by adapting the prompt tuning-based method, the entire LLM is frozen, and only a few learnable parameters of input embeddings are required to update to obtain satisfactory performance.
Therefore, we \xin{also} include the performance of \xin{DiscoPrompt} with the T5-11b version as a reference to explore the ability of a sizeable \jy{pre-trained} language model on this \xin{IDDR} task.
As shown in Table~\ref{tab:discourse relation classification PDTB 2.0} and Table~\ref{tab:discourserelation classification CoNLL16}, \xin{DiscoPrompt (T5-11b) easily beats other methods}, \xin{achieving} a 52.42\% F1 score and 68.14\% accuracy in the 11-class classification (second-level) task of the PDTB 2.0 (\textit{Ji}) and \xin{illustrating} the benefits without adjusting the representations from \xin{LLMs}.
\xin{
On the contrary, fine-tuning T5-11b is infeasible in most single compute nodes.
}

\begin{table*}[t]
\vspace{-0.6cm}
\centering
\small
  \scalebox{0.9}{\begin{tabular}{l| cc | cc | cc | cc }
    \toprule
    % \multirow{2}{*}{Data} &
    %   \multirow{2}{*}{ Models } &
    \multirow{2}{*}{ \textbf{Models} } &    % (CoNLL2016 Dataset)
    \multicolumn{2}{c|}{\textbf{Test (Top)}} &
    \multicolumn{2}{c|}{\textbf{Test (Second)}} &
    \multicolumn{2}{c|}{\textbf{Blind (Top)}} &
    \multicolumn{2}{c}{\textbf{Blind (Second)}}  \\
    %  \multicolumn{2}{c|}{\textbf{CoNLL-Test (Top)}} &
    % \multicolumn{2}{c|}{\textbf{CoNLL-Test (Second)}} &
    % \multicolumn{2}{c|}{\textbf{CoNLL-Blind (Top)}} &
    % \multicolumn{2}{c}{\textbf{CoNLL-Blind (Second)}}  &   
    % { } & {F1} & {Acc} & {F1}& {Acc} & {F1} & {Acc} & {F1} & {Acc} \\
    { } & {\textbf{F1}} & {\textbf{Accuracy}} & {\textbf{F1}}& {\textbf{Accuracy}} & {\textbf{F1}} & {\textbf{Accuracy}} & {\textbf{F1}} & {\textbf{Accuracy}} \\
    \midrule
    \cite{DBLP:conf/conll/WangL16} & - & - & - & 40.91 & - & - & - & 34.20 \\
    \cite{DBLP:conf/conll/RutherfordX16}& - & - & - & 36.13 & - & - & - & 37.67 \\
    \cite{Lan2017Multi} & - & - & - & 39.40 & - & - & - & 40.12 \\
    % \cite{Bai2018Deep} & - & - & - & -  & - & - & - & - \\
    % \cite{Xu2018Using} & - & - & - & - & -  & - & - & -\\
    % \cite{DBLP:conf/naacl/DaiH18} & - & - & - & - & - & - & - & -\\
    % \cite{DBLP:conf/acl/NguyenLTN19} & 53.00 & - & - & 49.95& - & - & - & 46.48\\
    % \cite{Dai2019A} & 52.89 & 59.66 & - & 48.23  & - & - & - & -\\
    % \cite{Shi2019Next}\footnotemark[2] & - & - & 53.23 (0.39) & - & - \\
    % \cite{Shi2019Next}\footnotemark[2] & - & - & - & 53.23 & - & - & - & - \\
    \cite{DBLP:conf/sigdial/VariaHC19} & - & - & - & 39.39 & - & - & - & 39.36 \\
    BMGF-RoBERTa~\cite{DBLP:conf/ijcai/LiuOSJ20}^*  & 56.55 & 68.23 & 40.68 & 57.26 & 58.30 & 74.43 & 28.98 & 55.19  \\    
    % LDSGM~\cite{DBLP:conf/aaai/WuCGLZS22} & 63.73 &  71.18 & 40.49 & 60.33 & - & - & - & - \\
    
    \midrule
    XLNet (base, cased)~\cite{DBLP:conf/acl/KimFGL20}^*  &  43.48 & 62.29 & 18.80 & 33.16 & 19.90 & 66.12 & 9.07 & 28.71 \\
    XLNet (large, cased)~\cite{DBLP:conf/acl/KimFGL20}^* & 47.07 & 64.76 & 27.13 & 47.85 & 22.37 & 66.59 & 11.94 & 35.06 \\
    T5-base(\jy{Fine-Tuning})~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}^* & 54.64 & 67.10 & 31.99 & 53.92  & 50.94 & 71.30 & 24.52 & 49.89 \\
    T5-large(\jy{Fine-Tuning})~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}^* & 58.74 & 70.87 & 34.66 & 58.88  & 56.28 & 73.07 & 24.63 & 54.30 \\
    \midrule
    Prefix-Tuning (T5-base)~\cite{DBLP:conf/acl/LiL20}^* & 26.18 & 55.35 & 8.26 & 26.63 & 27.17 & 65.88 & 9.70 & 32.71 \\
    Prefix-Tuning (T5-large)~\cite{DBLP:conf/acl/LiL20}^* & 57.84 & 71.15 & 46.06 & 59.40 & 55.61 & 74.12 & 30.53 & 55.53\\
    Prompt-Tuning (T5-base)~\cite{DBLP:conf/emnlp/LesterAC21}^* & 25.53 & 54.44 & 13.01 & 29.11 &  27.21 & 64.71 & 11.55 & 33.65\\
    Prompt-Tuning (T5-large)~\cite{DBLP:conf/emnlp/LesterAC21}^* & 59.95 & 72.32 & \underline{49.59} & \underline{60.57} & 63.35 & \underline{77.41} & \underline{35.72} & \underline{57.88}\\
    % Prompt Tuning (T5-large)~\cite{DBLP:conf/emnlp/LesterAC21} & 59.95 & 72.32 & \underline{49.59} & \underline{60.57} & 61.08 & \underline{78.12} & \underline{36.27} & \underline{59.53}\\
    % PCP w/ RoBERTa-base~\cite{DBLP:journals/corr/abs-2210-07032} & - & - & - & 60.98  & - & -  & - & 57.31\\     
    PCP (RoBERTa-base)~\cite{DBLP:journals/corr/abs-2210-07032}^* & 58.54 & 69.31 & 33.27 & 55.48 & 55.30 & 72.00  & 26.00 & 50.99 \\
    % PCP w/ RoBERTa-large~\cite{DBLP:journals/corr/abs-2210-07032} & - & - & - & \underline{63.36}  & - & -  & - & 58.51\\    
    PCP (RoBERTa-large)~\cite{DBLP:journals/corr/abs-2210-07032}^* & \underline{63.78} & \underline{72.69} & 37.79 & 58.36 & \underline{64.74} & 76.47  & 27.77 & 56.24 \\   
    \midrule
    % \bf DiscoPrompt (T5-base) & 58.71 & 70.50 & 43.18 & 57.31 & 55.24 & 73.88 & 31.98 & 55.53 \\
    % \bf DiscoPrompt (T5-large) &  67.81 &  74.41 & 50.52 &  64.88 &  63.61 & 77.41 & 34.31 & 60.71\\
    DiscoPrompt (T5-base) & 60.66 & 70.63 & 45.99 & 60.84  & 62.98 &  76.94 &  39.27 & 57.88\\
    DiscoPrompt (T5-large) & \bf 69.56 & \bf 75.33 & \bf 56.29 & \bf 66.32 & \bf 67.89 & \bf 80.47 & \bf 38.49 & \bf 63.06\\
    % \bf DiscoPrompt (t5-v1\_1-large) & \bf 69.56 & \bf 75.33 & \bf 56.29 & \bf 66.32 & \bf 66.43 & \bf 80.00 & \bf 37.61 & \bf 64.47\\
    \midrule
    % \bf DiscoPrompt (t5-v1\_1-xl) & 70.92 & 76.76 & 56.34 & 68.54 & 73.39 &  82.59 &  40.68 &  63.76\\
    DiscoPrompt (T5-11b) & 70.38 & 78.07 & 57.75 & 69.71  & 72.33 & 84.94 & 38.60 & 66.35\\ 
    \bottomrule
  \end{tabular}}
  \vspace{-0.05in}
  \caption{
  \label{tab:discourserelation classification CoNLL16}
The accuracy (\%) and F1 score (\%) are evaluated on the implicit discourse partition of CoNLL2016 dataset. * represent the implemented and reproduced model performance.
}
\vspace{-0.5cm}
\end{table*}




% \textbf{Third}, the performance of prompt tuning-based methods relies on the model scale, consistent with previous works~\cite{DBLP:conf/eacl/SchickS21,DBLP:conf/emnlp/LesterAC21,DBLP:conf/acl/0010LLWWBCH22}, especially the prefix-tuning and prompt-tuning methods.
% \paragraph{PTBD 2.0 Performance}
% Table~\ref{tab:discourse relation classification PDTB2.0} summarizes the main results of the PDTB 2.0 Ji and Lin settings, from which we derive the following conclusions. \textbf{First}, our method significantly outperforms all baselines and achieves state-of-the-art performance on this task at both top-level and second-level classes. Specifically, our method gains a considerable improvement of 6.93\% second-level accuracy, 10.99\% second-level F1 score, 5.96\% top-level accuracy, and 9.47\% top-level F1 score over the T5-large fine-tuning in PDTB 2.0-JI setting. \textbf{Second}, the prompt-based baselines can receive an outstanding performance on this task. It may attribute to prompt-based methods being effective in utilizing the training data instances (shown in many previous works~\cite{DBLP:conf/acl/LiL20,DBLP:conf/emnlp/LesterAC21}), and the data amount of the original training set is insufficient for fine-tuning all parameters of pre-train language models to generalized to the test set. \textbf{Third}, the performance of prompt tuning-based methods relies on the model scale, consistent with previous works~\cite{DBLP:conf/eacl/SchickS21,DBLP:conf/emnlp/LesterAC21,DBLP:conf/acl/0010LLWWBCH22}, especially the Prefix-Tuning and Prompt Tuning methods. \textbf{Fourth}, the ContrastiveIDRR and our method obtain a better performance on the F1 score evaluation metric. It may result from adopting the hierarchy label information and dependence among the top-level and second-level senses.

% \paragraph{CoNLL2016 Performance}
% Table~\ref{tab:discourserelation classification CoNLL16} reports the main experimental results of the CoNLL2016 test and Blind set. Our method consistently delivers the new SOTA performance with substantial improvements over all baselines on the CoNLL2016 dataset in the implicit discourse relation recognition task. Our model received a significant improvement of 8.76\% second-level accuracy, 13.86\% second-level F1 score, 7.4\% top-level accuracy, and 11.61\% top-level F1 score over T5-large fine-tune in this CoNLL16 Blind set. It demonstrates that our method effectively utilized the hierarchy information and mined specific knowledge on the correlation of discourse relation and connectives for improving the generalization ability of the T5 model to undertake this task. An interesting finding is that the original prompt tuning method (with T5-large) obtained better performance than the T5-large fine-tune method. This situation may be because the T5-large model tends to overfit the small amount of training set by fine-tuning all learnable parameters of the model. In contrast, the prompt tuning method is better at effectively utilizing the data instances and only tunes on extremely few tunable parameters. The learnable parameters of baselines and our model are shown in Appendix~\ref{sec:appendix_approximation_learnable parameters}.

 


% \paragraph{CoNLL2016 Performance}
% Table~\ref{tab:discourserelation classification CoNLL16} reports the main experimental results of the CoNLL2016 test and Blind set. We observe that our method consistently delivers the new SOTA performance with substantial improvements over all baselines on the CoNLL2016 dataset of the implicit discourse relation recognition task. Our model received a significant improvement of 4.34\% second-level accuracy, 11.24\% second-level F1 score, 4.31\% top-level accuracy, and 6.18\% top-level F1 score over T5-large fine-tune in this CoNLL16 Blind set. It demonstrates that our method effectively utilized the hierarchy information and mined specific knowledge on the discourse relation and connectives for improving the generalization ability of the T5 model to undertake this task. An interesting finding is that the Prompt tuning method (with T5-large) obtained a better performance on many evaluation metrics except for the top-level F1 score compared with the T5-large fine-tune method. The reason behind this situation may be the T5-large model fine-tunes all tunable parameters of the model and tend to overfit on the small amount of training set, while the prompt tuning method only tunes on extremely few tunable parameters and perform well on low data regime. The tunable parameters of baselines and our model are shown in Table~\ref{tab:tunable_parameters} in Appendix.

% In this paper, we are also interested in the large pre-train language model that will receive what performance on this task. 
% Fine-tuning a pre-train language model such as T5-3b and T5-11b required extensive computation machines to update all trainable parameters of the whole pre-train language model. However, by adapting the prompt-tuning based method, we only need to update the few learnable parameters of the model input. Therefore, we implement our method adopting the T5 with the 11B version to train the tunable parameter from model input and get the performance as a reference to notify us of the ability of a large pre-train language model on this implicit discourse relation recognition task.

% \section{Analysis}
% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{lc c c }
% \hline
% \textbf{Model} & \textbf{Top-Sec} & \textbf{Top-Sec-Con}
% \hline
% HierMTN-CRF & 46.29 & 19.15\\
% BMGF-RoBERTa & 47.06 & 21.37\\
% % OurEncoder+OurDecoder & 57.86 & 25.31
% LDSGM & 58.61 & 26.85\\
% % DiscoPrompt  & \textbf{96.73} & \textbf{95.64}\\ 
% \hline
% \end{tabular}
% \vspace{-0.05in}
% \caption{
% Comparison with recent models on the consistency
% among multi-level label predictions.
% }
% \label{tab:EDRR_Performance}
% \end{table}

\begin{table*}[!htbp]
\vspace{-0.6cm}
\small
\centering
\scalebox{0.9}{\begin{tabular}{l|c|c|c|c}
\toprule
\multicolumn{1}{c|}{\textbf{Model}}
& \textbf{Top(F1)} & \textbf{Top(Acc)} & \textbf{Sec(F1)} & \textbf{Sec(Acc)} \\
\midrule
DiscoPrompt(T5-large) & \textbf{70.84} & \textbf{75.65} & \textbf{49.03} & \textbf{64.58} \\
\midrule
   % w/ Top and Second Level  Mask  & 53.93 & 66.89 & 33.74 & 53.71\\
   % w/ Top Level and Connective Mask & 69.19 & 72.57 & 42.95 & 64.08\\
   % w/ Second Level and Connective Mask & 70.04 & 74.69 & 45.98 & 64.37\\
   % w/ Connective Mask & 68.00 & 73.82 & 43.76 & 63.43 \\
   w/ Path (Top-Second Level Mask)  & 53.93 & 66.89 & 33.74 & 53.71\\
   w/ Path (Top-Connective Mask) & 69.19 & 72.57 & 42.95 & 64.08\\
   w/ Path (Second-Connective Mask) & 70.04 & 74.69 & 45.98 & 64.37\\
   w/ Path (Connectives Mask) & 68.00 & 73.82 & 43.76 & 63.43 \\
% \midrule
%    Continuous Prompt Length (10) & 67.17 & 72.47 & 43.56 & 62.66\\
%    Continuous Prompt Length (50) & 69.64 & 74.40 & 45.06 & 63.91\\
%    Continuous Prompt Length (100) & 68.39 & 73.92 & 42.77 & 64.20\\
\midrule
  w/o Entire Discrete Prompt & 68.38 & 72.95 & 41.79 & 62.66 \\ 
  w/o Cloze Discrete Prompt & 68.64 & 73.72 & 41.44 & 63.72 \\
  w/o Hierarchy Tree Prompt & 68.03 & 72.18 & 43.14 & 62.85\\
\midrule
  w/ Continuous Hierarchy Prompt  & 67.63 & 73.24 & 44.03 & 63.81 \\
  w/ Continuous Labels \& Connective & 67.74  & 73.24 & 44.06 & 64.10 \\
  w/ Continuous Connective & 68.35  & 73.15 & 44.48 & 64.20 \\  
\bottomrule
\end{tabular}}
\vspace{-0.05in}
\caption{
Performance of ablation study in our method DiscoPrompt (T5-large) on PDTB 2.0-Ji dataset. The path prediction of DiscoPrompt has three levels of masks containing top-level class, second-level class, and connectives mask (e.g., `` Path (Connectives Mask)'' indicates only one mask in our predicted path for predicting the connectives and mapping to label). The entire discrete prompt in our template includes the cloze discrete prompt and the hierarchy tree prompt. The last partition of the table is the ablation study on the  discrete hierarchy tree prompt to gradually replace the discrete tokens with continuous ones in various parts.
% ``Top and Second Level Mask'' means our method with only two masks for receiving the top-level and second level likelihood.
}
\label{table:methods_ablation}
\vspace{-0.6cm}
\end{table*}


\subsection{Ablation Study}
% In this section, we investigate the factors that influence the performance of our model, which includes the ablation study on our path prediction model and the tailored hierarchical tree prompt.
\xin{
To better investigate the factors of DiscoPrompt, we design numerous ablations on the path prediction and the tailored hierarchical tree prompt.
}
Table~\ref{table:methods_ablation} reports the performance of the ablation study for our model in the PDTB 2.0 (\textit{Ji}).

\paragraph{Mask Number in Path Prediction}
In our method, by estimating the \xin{likelihoods} of $p_1^j$ (the top-level), $p_2^j$ (the second-level), and $p_3^j$ (the connective) in a predicted path, the dependencies of these three masks were utilized for enhancing the ability of the \jy{pre-trained} language model on this IDRR task.
According to the experimental result in Table~\ref{table:methods_ablation}, we can conclude that 1) the performance of the path prediction model incorporating the signals from all three masks surpasses other models,  which path forming by only two masks or even one connectives mask.
This result emphasizes the significance of the information and dependencies among these marks in our path prediction model; 2) the predicted path model without prior knowledge of selected connectives performs worst, which is consistent with findings in~\citet{DBLP:journals/corr/abs-2210-07032}; 3) the predicted path model with only connective mask performs worse than incorporating the prior knowledge of connectives with the top-level class or second-level class information.
It highlighted the importance of intrinsic senses of label words to help the pre-trained language model understand the task.



% 3) although the predicted path model (with second-level label and connectives mask) obtains an \jy{excellent} performance on this task, this performance can be further improved by integrating the top-level class information.
% \paragraph{Continuous Prompt Length}
% The continuous prompt (i.e., learnable prompt tokens) length is another factor that influences the performance of our model. Hence, we implement various prompt lengths of 10, 20, 50, and 100. The optimal continuous prompt length is 20, which provides the best performance among all the prompt lengths and is the default prompt length for implementing other experiments. Adopting more prompt length than 20 on our method will not significantly increase this task's performance on various evaluation metrics. 

\paragraph{Discrete Prompt Template} Two portions in our designed prompt template are in natural textual form and as a discrete non-tunable token. The first part is the discrete tokens for the label hierarchy structure (i.e., hierarchy tree prompt), shown in Figure~\ref{fig:DiscoPrompt_Template_Searching}. The second part is the cloze discrete prompt `` The path is ''. The performance shown in Table~\ref{table:methods_ablation} demonstrates that these \jy{two parts} of the prompt \jy{are} essential for achieving satisfactory performance compared with the without these two parts (i.e., w/o Entire Prompt). Without injects structural information from the explicitly hierarchical tree prompt, the performance dropped significantly, especially the second-level F1 score, dropping from 49.03\% to 43.14\% F1 score.

% There are two portions of prompts in natural textual form and as a discrete non-tunable token in our designed prompt template. The first part is the prompt for the senses label hierarchy structure which demonstrates in Figure~\ref{fig:DiscoPrompt_Template_Searching}. The second part is the cloze discrete prompt `` The path is ''.  The performance shown in Table~\ref{table:methods_ablation} demonstrates that these two part of the prompt is essential for achieving good performance compared with the without these two part of the prompt (i.e., w/o Whole Prompt). Without the sense label hierarchy prompt, the performance drop significant, especially the second-level F1 score drop from 49.03\% to 43.14\% F1 score. 



% \begin{table*}[!htbp]
%     \small
%     \centering
%     \begin{tabular}{l|c|c|c|c}
%     \toprule
%     \multicolumn{1}{c|}{\textbf{Model}}
%     & \textbf{Top(F1)} & \textbf{Top(Acc)} & \textbf{Sec(F1)} & \textbf{Sec(Acc)} \\
%     \midrule
%     DiscoPrompt (T5-large) & \textbf{70.84} & \textbf{75.65} & \textbf{49.03} & \textbf{64.58} \\
%     \midrule
%       w/ Continuous Hierarchy Prompt  & 67.63 & 73.24 & 44.03 & 63.81 \\
%       w/ Continuous Labels \& Connective & 67.74  & 73.24 & 44.06 & 64.10 \\
%       w/ Continuous Connective & 68.35  & 73.15 & 44.48 & 64.20 \\  
%       w/o Hierarchy Prompt & 68.03 & 72.18 & 43.14 & 62.85\\
%     \bottomrule
%     \end{tabular}
%     \vspace{-0.05in}
%     \caption{Performance of various hierarchy prompt settings in DiscoPropmt (T5-large) in PDTB2.0-Ji dataset.}
%     \vspace{-0.1cm}
%     \label{table:hierarchy_tree_ablation}
% \end{table*}

% \subsubsection{Ablation Study on Sense Label Hierarchy Prompt}
\paragraph{Hierarchical Tree Prompt}
To acquire a deeper understanding of the discrete hierarchy tree prompt, we perform experiments to gradually replace the discrete tokens with continuous ones in various elements of this hierarchy prompt. The experiments include 1) replacing the whole hierarchy tree prompt as the continuous tunable prompt with the same number of tokens, 2) only including the ``-> ''  and replacing other relation labels and connective as continuous tunable prompt, and 3) \jy{only replacing} the textual connective to be the tunable prompt. The experimental result in Table~\ref{table:methods_ablation} underscores the importance and effectiveness of our tailored discrete hierarchy tree prompt is higher than the continuous learnable searched template. 


% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{l|c|c|c|c}
% \toprule
% \multicolumn{1}{c|}{\textbf{Model}}
% & \textbf{Top(F1)} & \textbf{Top(Acc)} & \textbf{Sec(F1)} & \textbf{Sec(Acc)} \\
% \midrule
% DiscoPrompt (Optimal Template : The path is {mask} -> {mask};) & \textbf{70.84} & \textbf{75.65} & \textbf{49.03} & \textbf{64.58} \\
% \midrule
% DiscoPrompt (Template 1: The path is {mask} -> {mask} -> {mask}) & 69.22 & 73.44 & 43.52 & 63.33 \\
% DiscoPrompt (Template 2: The relation is {mask}.{mask}) & 67.55  & \underline{74.21} & 44.81 & \underline{64.20}  \\
% DiscoPrompt (Template 3: The relation is {mask} -> {mask})& \underline{69.70} & 74.01 & \underline{48.61} & 64.10\\
% DiscoPrompt (Template 4: The relation is {mask} -> {mask} -> {mask};) & 68.07 & 72.76 & 45.91 & 62.56 \\
% DiscoPrompt (Template 5: The relation is {mask} -> {mask}.The connective is {mask} .) & 62.71 & 70.74 & 40.19 & 58.81 \\
% \bottomrule
% \end{tabular}
% \vspace{-0.05in}
% \caption{Performance of various template of our method with adopting T5-large model in PDTB2.0-Ji dataset.The details of various template shown in Figure~\ref{table:Prompt_Template_Searching} in Appendix.}
% \vspace{-0.3cm}
% \label{table:Prompt_Template_Searching}
% \end{table*}

\paragraph{Prompt Engineering} Furthermore, we implement the prompt template searching and the \xin{parameter sensitivity} on the continuous prompt length, \xin{which we describe in Appendix~\ref{sec: Appendix_ablation_study_DiscoPrompt}}.
% The performance and prompt template details are in Appendix~\ref{sec: Appendix_ablation_study_DiscoPrompt}. 


\begin{table}[t]
\small
\centering
\scalebox{0.85}{\begin{tabular}{l|c|c|c|c}
\toprule
\multicolumn{1}{c|}{\textbf{Model}}
& \textbf{Comp.} & \textbf{Cont.} & \textbf{Exp.} & \textbf{Temp.} \\
\midrule
\cite{DBLP:conf/acl/NguyenLTN19} & 48.44 & 56.84 & 73.66 & 38.60\\
\cite{DBLP:conf/aaai/GuoHDW20} & 43.92 & 57.67 & 73.45 & 36.33\\
\cite{DBLP:conf/ijcai/LiuOSJ20} & 59.44 & 60.98 & 77.66 & 50.26 \\
\cite{DBLP:conf/emnlp/JiangFCLZ21} & 55.40 & 57.04 & 74.76 & 41.54\\
\cite{DBLP:conf/emnlp/DouHSZ21} & 55.72 & 63.39 & 80.34 & 44.01\\
\cite{conf/emnlp/Contrastive_Learning} & 65.84 & 63.55 & 79.17 & \underline{69.86}\\
\hline
% DiscoPrompt (T5-base)& 56.06 & 65.33 & 78.12 & 57.66 \\
% DiscoPrompt (T5-large)& \bf65.08 & \bf67.78 & \bf81.26 & \bf57.69 \\
DiscoPrompt (T5-base)& 62.55  & 64.45  & 78.77 & 57.41 \\
DiscoPrompt (T5-large)& \underline{67.13}  & \underline{69.76} & \underline{81.61} & 64.86 \\
% DiscoPrompt (T5-large)& \bf67.91   & \bf67.67  & \bf81.06  & \bf71.70  \\
\hline
DiscoPrompt (T5-11B)& \bf74.35  & \bf 72.44 & \bf82.57 & \bf72.00 \\
\bottomrule
\end{tabular}}
\vspace{-0.05in}
\caption{The performance for top-level classes on PDTB 2.0-Ji in terms of F1 (\%) (top-level multi-class classification). More baselines for comparison can be found in Table~\ref{table:appendix_binary} in Appendix~\ref{sec:appendix_Performance on Top and Second level}.}
\label{table:binary}
\vspace{-0.6cm}
\end{table}

\begin{table}[t]
\small
\centering
\scalebox{0.85}{\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Second-level Label}  & \textbf{PCP} & \textbf{Contrast.}  & $\textbf{Ours}_{(\textbf{large})}$ & $\textbf{Ours}_{(\textbf{11B})}$ \\
\midrule
\textit {Temp.Asynchronous} & 57.81 & 59.79  & 64.15 & \bf72.27\\
\textit {Temp.Synchrony} & 0.0 & \bf78.26 & 50.00 & 33.33\\
\hline
\textit {Cont.Cause} &  65.64 & 65.58  & 69.66 & \bf72.28\\
\textit {Cont.PragmaticCause} & 0.0 & 0.0 & 0.0 & 0.0\\
\hline
\textit {Comp.Contrast}  & 63.88 & 62.63 &  62.88 & \bf70.63\\
\textit {Comp.Concession}  & 8.00 & 0.0 & \bf 9.09 & 0.0 \\
\hline
\textit {Expa.Conjunction} & 57.78 & 58.35 &  60.09 & \bf62.84\\
\textit {Expa.Instantiation} & 74.01 & 73.04  & 74.17 & \bf76.60\\
\textit {Expa.Restatement} & 61.00 & 60.00 & 65.24 & \bf 65.98\\
\textit {Expa.Alternative} & 66.67 & 53.85  &  60.00 & \bf84.21\\
\textit {Expa.List} & 29.63 & 34.78 & 24.00 & \bf38.46\\
\bottomrule
\end{tabular}}
\vspace{-0.05in}
\caption{The label-wise F1 scores for the second-level labels on PDTB2.0-Ji (second-level multi-class classification). More baselines is in Table~\ref{table:Appendix_Label_wise_F1} in Appendix~\ref{sec:appendix_Performance on Top and Second level}. `` Contrast.'' indicate the ContrastiveIDRR~\cite{conf/emnlp/Contrastive_Learning} baseline.}
\vspace{-0.6cm}
\label{table:Label-wise F1}
\end{table}

\subsection{Label-wise F1 Score on Top-Level and Second-level}
The PDTB 2.0-Ji setting exhibits a highly skewed label distribution, with only roughly 854 training instances (i.e., 6.8\% of 12406 training instances) annotating as five of the 11 second-level labels. To further explore our model in four top-level relations and 11 second-level sense types on this dataset, Table~\ref{table:binary} and Table~\ref{table:Label-wise F1} reported the F1 score (\%) in the top-level and second-level classes, respectively. In Table~\ref{table:binary}, our model outperforms all baselines in three top-level relations (i.e., \textit{Comparison}, \textit{Contingency}, \textit{Expansion}), and most of the baselines in the \textit{Temporal} relation except ContrastiveIDRR. Specifically, Table~\ref{table:Label-wise F1} illustrates that our model performs better on the \textit{Temp.Asynchronous} second-level class, whereas ContrastiveIDRR performs well on the \textit{Temp.Synchrony}. In Table~\ref{table:Label-wise F1}, our model obtains a valid F1 score in most second-level classes but the \textit{Cont.Pragmatic Cause} class still are 0\% F1 score same as all baselines. This situation may result from the few training examples of this class being insufficient for optimal learnable parameters, and the model tends to ignore this class in the prediction process. However, our model obtained a 50.0\% F1 score and 9.09\% F1 score in another two second-level classes with less training data (i.e., \textit{Temp.Synchrony}, \textit{Comp.Concession}), while PCP received 0\% F1 score in \textit{Temp.Synchrony} class and ContrastiveIDRR acquire 0\% F1 score in \textit{Comp.Concession} class. 
% This performance may attribute to our method utilizing the hierarchical structural information and prior knowledge regarding the connectives.




% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{l|c|c|c|c}
% \toprule
% Second-level Label& BMGF-RoBERTa & LDSGM & DiscoPrompt_{(base)} & DiscoPrompt_{(large)}  \\
% \midrule
% \textit {Temp.Asynchronous} & 56.18 & 56.47 & 57.94 & \bf58.59\\
% \textit {Temp.Synchrony} & 0.0 & 0.0 & 0.0 & \bf40.00\\
% \hline
% \textit {Cont.Cause} & 59.60 & 64.36 & 65.08  & \bf 67.42\\
% \textit {Cont.Pragmatic cause} & 0.0 & 0.0 & 0.0 & 0.0 \\
% \hline
% \textit {Comp.Contrast} & 59.75 & 63.52 & 55.28 & \bf 59.50\\
% \textit {Comp.Concession} & 0.0 & 0.0 & \bf 11.11 & 0.0 \\
% \hline
% \textit {Expa.Conjunction} & 60.17 & 57.91 &  59.67 & \bf 62.32\\
% \textit {Expa.Instantiation} & 67.96 & 72.60 & 68.93 & \bf 71.71\\
% \textit {Expa.Restatement} & 53.83 & 58.06 & 57.40 & \bf64.53 \\
% \textit {Expa.Alternative} & 60.00 & 63.46 &  63.64 & \bf 70.59\\
% \textit {Expa.List} & 0.0 & 8.98 & \bf 38.10 & \bf38.10\\
% \bottomrule
% \end{tabular}
% \caption{Label-wise F1 scores for the second-level labels.}
% \label{table:Label-wise F1}
% \end{table*}

% \begin{table*}[t]
% \small
% \centering
% \scalebox{0.9}{\begin{tabular}{l|c|c|c|c|c|c|c}
% \toprule
% \textbf{Second-level Label} & \textbf{BMGF} & \textbf{LDSGM} & \textbf{PCP} & \textbf{ContrastiveIDRR} & $\textbf{Ours}_{(\textbf{base})}$ & $\textbf{Ours}_{(\textbf{large})}$ & $\textbf{Ours}_{(\textbf{11B})}$ \\

% % Second-level Label& BMGF-RoBERTa & LDSGM & PCP-large & DiscoPrompt_{(base)} & DiscoPrompt_{(large) & DiscoPrompt_{(11B)}  \\
% % Second-level Label & \cite{DBLP:conf/ijcai/LiuOSJ20} & \cite{DBLP:conf/aaai/WuCGLZS22} & \cite{DBLP:journals/corr/abs-2210-07032}  & DiscoPrompt_{(base)} & DiscoPrompt_{(large) & DiscoPrompt_{(11B)}  \\
% \midrule
% \textit {Temp.Asynchronous} & 56.18 & 56.47 & 57.81 & 59.79 & 57.69 & 64.15 & \bf72.27\\
% \textit {Temp.Synchrony} & 0.0 & 0.0 & 0.0 & \bf78.26 & 0.0 & 50.00 & 33.33\\
% \hline
% \textit {Cont.Cause} & 59.60 & 64.36 & 65.64 & 65.58 & 63.83  &  69.66 & \bf72.28\\
% \textit {Cont.PragmaticCause} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
% \hline
% \textit {Comp.Contrast} & 59.75 & 63.52 & 63.88 & 62.63 & 59.26  &  62.88 & \bf70.63\\
% \textit {Comp.Concession} & 0.0 & 0.0 & 8.00 & 0.0 & \bf 9.09 & \bf 9.09 & 0.0 \\
% \hline
% \textit {Expa.Conjunction} & 60.17 & 57.91 & 57.78 & 58.35 &  61.08 &  60.09 & \bf62.84\\
% \textit {Expa.Instantiation} & 67.96 & 72.60 & 74.01 & 73.04 & 69.96 & 74.17 & \bf76.60\\
% \textit {Expa.Restatement} & 53.83 & 58.06 & 61.00 & 60.00 & 58.45 & 65.24 & \bf 65.98\\
% \textit {Expa.Alternative} & 60.00 & 63.46 & 66.67 & 53.85 & 72.73 &  60.00 & \bf84.21\\
% \textit {Expa.List} & 0.0 & 8.98 & 29.63 & 34.78 &  37.50 & 24.00 & \bf38.46\\
% \bottomrule
% \end{tabular}}
% \vspace{-0.05in}
% \caption{The label-wise F1 scores for the second-level labels on PDTB2.0-Ji(second-level multi-class classification).}
% \vspace{-0.3cm}
% \label{table:Label-wise F1}
% \end{table*}


\subsection{Designed Prompt For T5 \jy{Fine-Tuning}} \label{sec:Designed Prompt For T5 Fine-Tuning}
To demonstrate the effectiveness of our designed template and explore whether our designed template can be used for the \jy{fine-tuning} paradigm, we convert the data input to the tailored prompt template in Figure~\ref{fig:DiscoPrompt_Template_Searching} in Appendix but with only a [MASK] for generating the entire path and feed to the T5-large model for fine-tuning on CoNLL16 dataset. The experimental result is summarised in Figure~\ref{fig:T5_finetune_template_CoNLL2016}, and all models gain certain improvements over vanilla T5-large fine-tuning. The overall improvement obtained around one to two points accuracy or F1 score, which illustrates the effectiveness of our tailored template. The detailed performance is shown in Table~\ref{table:T5-large-fine-tune-template-table}, and the experimental result for PDTB2.0 is shown in Figure~\ref{fig:T5_finetune_template_PDTB2.0} in Appendix~\ref{appendix_Performance of Designed Prompt For T5 Fine-Tune}.




\begin{figure}[t]
    \vspace{-0.8cm}
    \centering
    \includegraphics[width=\linewidth]{sections/Figures/T5_template.pdf}
    \vspace{-0.25in}
    \caption{The performance comparison of the T5-large fine-tuning with and without using our designed template on the CoNLL16 dataset. ``T5-templ.''means adapting our template to the fine-tuning paradigm. Acc and F1 inside the brackets indicate the accuracy and F1 score. 
    }
    \label{fig:T5_finetune_template_CoNLL2016}
    \vspace{-0.3cm}
\end{figure}

\begin{table}[!t]
\vspace{-0.1cm}
\small
\centering
\begin{tabular}{lc c c }
\hline
\textbf{Model} & \textbf{Acc (\%)} & \textbf{F1(\%)}\\
\hline
% Connective Only~\cite{DBLP:conf/acl/PitlerN09}      & 93.67 & - \\ 
% % +Syntax+Conn-Syn~\cite{DBLP:conf/acl/PitlerN09}     & 94.15 & - \\ 
% Syntax+Conn~\cite{DBLP:conf/acl/PitlerN09}     & 94.15 & - \\ 
% ELMo-C\&E~\cite{Dai2019A}                           & 95.39 & 94.84\\
% PEDRR~\cite{DBLP:journals/corr/abs-2210-07032}      & 94.78 & 93.59\\
% RWP-CNN~\cite{DBLP:conf/sigdial/VariaHC19}          & 96.20 & 95.48\\ 
% \hline
% \cite{DBLP:conf/acl/PitlerN09}      & 93.67 & - \\ 
\cite{DBLP:conf/acl/PitlerN09}     & 94.15 & - \\ 
\cite{DBLP:conf/naacl/DaiH18}  & 94.46 & 93.70 \\
\cite{Dai2019A}                           & 95.39 & 94.84\\

\cite{DBLP:journals/corr/abs-2210-07032}      & 94.78 & 93.59\\
\cite{DBLP:conf/sigdial/VariaHC19}          & 96.20 & 95.48\\ 
\hline 
% DiscoPrompt (Ours)                                  & 96.00 & 94.93\\
T5-large (\jy{fine-tuning}) (w/o connective) & 74.47 & 72.38\\ 
T5-large (\jy{fine-tuning}) (w/ connective)& 95.41 & 94.94\\ 
DiscoPrompt (w/ connective mask) & 78.35 & 74.62\\
DiscoPrompt (w/ true connective )  & \textbf{96.73} & \textbf{95.64}\\ 
\hline
\end{tabular}
\vspace{-0.1in}
\caption{
Experimental results on PDTB 2.0 Top-level senses for EDRR. ``w/o connective '' represent without using the provided connectives in the EDRR task.
}
\label{tab:EDRR_Performance}
\vspace{-0.6cm}
\end{table}

\subsection{Generalization to Explicit Discourse Relation Classification Task}\label{sec:generalizationEDRR}
To demonstrate the generalization ability of our model, we transfer and adapt our method to the explicit discourse relation recognition (EDRR) task. We want to explore the ability of our model on this task given annotated connectives. Our prompt template only replaces the first [MASK] position between two arguments as the given connectives from each data instance in the EDRR task. Following the previous works~\cite{DBLP:conf/sigdial/VariaHC19, DBLP:journals/corr/abs-2210-07032}, the second-level class is the same as our implicit one setting. In Table~\ref{tab:EDRR_Performance}, our model slightly outperforms previous SOTA models on the top-level senses in PDTB 2.0 dataset. This performance demonstrated the generalization ability of our method on the EDRR task.

\begin{table}[!t]
\vspace{-0.6cm}
\small
\centering
\scalebox{0.85}{\begin{tabular}{l|c|c|c|c}
\toprule
\multicolumn{1}{c|}{\textbf{Model}}
& \textbf{Top(F1)} & \textbf{Top(Acc)} & \textbf{Sec(F1)} & \textbf{Sec(Acc)} \\
\hline
Random & 23.44 & 32.18 & 6.48 & 8.78 \\
% Label only  & 43.37 & 48.51 & 16.17 & 26.95  \\
% Label+Connective & - & - & -& -\\
% In Context & - & - & -& -\\
% Structure & 44.09 & 50.24 & 19.88 & 31.95 \\

ChatGPT$_{label}$ & 43.37 & 48.51 & 16.17 & 26.95  \\
ChatGPT$_{label \& con.}$ & 43.99 & 49.28 & 17.55& 30.32\\
ChatGPT$_{structure}$ & 44.09 & 50.24 & 19.88 & 31.95 \\
\hline
\end{tabular}}
\vspace{-0.1in}
\caption{
The performance of ChatGPT performs on the PDTB 2.0-Ji test set. ChatGPT$_{label \& con.}$ means predicting the label and connective, and ChatGPT$_{structure}$ means adopting our structural path prompt template.
}
\label{tab:ChatGPT_Performance}
\vspace{-0.7cm}
\end{table}

\subsection{Zero-Shot With ChatGPT}
With the powerful ability of LLM and ChatGPT exhibited on numerous tasks, we are curious about the capability of ChatGPT on this IDRR task. We test the ability of ChatGPT with three designed templates on the PDTB2.0-Ji test set, and the performance is shown in Table~\ref{tab:ChatGPT_Performance}. In Table~\ref{tab:ChatGPT_Performance}, all designed templates obtain a performance higher than the random, but still at a low region in the second-level class compared with the supervised setting. This result demonstrates that the IDRR task is difficult for ChatGPT and cannot solve easily. The structural path template outperformed another two templates and proved that the structural form of the template is helpful for ChatGPT to understand this task. The F1 score of each second level is shown in Figure~\ref{fig:appendix_ChatGPT_performance_figure} in Appendix and illustrates that the path structure template is effective for ChatGPT to distinguish various second-level senses among \textit{Expansion} top class. The case examples and more discussion is in Appendix~\ref{sec:appendix_Discussion for ChatGPT and Case Example}.



% The F1 score of each second level is shown in Figure~\ref{fig:appendix_ChatGPT_performance_figure} in Appendix. The case examples and more discussion is in Appendix~\ref{sec:appendix_Discussion for ChatGPT and Case Example}.




% More discussion is in the Appendix~\ref{sec:appendix_Discussion for ChatGPT and Case Example}.

% These templates include: 1) predict the class label only, 2) predict the class label with connectives, and 3) predict the class label with connectives in a structural path form. 
% An interesting finding is that the ChatGPT with label-only template tends to predict many temporally related instances to the \textit{Contingency.Cause} second-level sense result in poor performance on \textit{Temporal.synchrony} second-level sense. More details of input templates and case examples are shown in Appendix~\ref{sec:appendix_ChatGPT_case_study}.





% With the powerful ability of LLM and ChatGPT exhibited on numerous tasks, we are curious about the capability of ChatGPT on the PDTB2.0-Ji test set. ChatGPT\footnotemark[7] employs the same approaches as InstructGPT~\cite{DBLP:journals/corr/abs-2203-02155}, which uses the GPT-3.5 as the backbone model trained to follow the instruction in a prompt and provide a thorough answer, but with slight modifications in the data collection setup. We test the ability of ChatGPT with three templates on the PDTB2.0-Ji test set, and the performance is shown in Table~\ref{tab:ChatGPT_Performance}. These templates\footnotemark[8] include: 1) predict the class label only, 2) predict the class label with connectives, and 3) predict the class label with connectives in a structural path form. In Table~\ref{tab:ChatGPT_Performance}, all designed templates obtain a performance higher than the random, but still at a low region in the second-level class compared with the supervised setting. This result demonstrates that the IDRR task is difficult for ChatGPT and cannot solve easily. The structural path template gained improvement over another two templates and proved that the structural form of the template is helpful for ChatGPT to understand this task. The F1 score of each second level is shown in Figure ~\ref{fig:ChatGPT_performance_figure} and illustrates that the path structure template is effective for ChatGPT to distinguish various second-level senses among \textit{Expansion} top class. An interesting finding is that the ChatGPT with label-only template tends to predict many temporally related instances to the \textit{Contingency.Cause} second-level sense result in poor performance on \textit{Temporal.synchrony} second-level sense. More details of input templates and case example are shown in Appendix~\ref{sec:appendix_ChatGPT_case_study}.


% ChatGPT not only predict the answer, but also offer more details why generate this answer.  % a good example (Expansion) and a bad example (Temporal.synchrony),

% Although we provide a in-context learning template for ChatGPT, it still perform same as original label prediction one. With in-context learning, they tends to state more class but accuracy is still low. 
% In-context learning~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} provide a few training examples (a list of input-output pairs) as its context with a test instance to be the input feed to a large pretrained language model (LM) for directly decoding the output without any update to its parameters.

% \footnotetext[7]{The demonstration and details of ChatGPT are on the website \url{https://openai.com/blog/chatgpt/}}
% \footnotetext[8]{The input template with in-context learning highly relies on the training examples selected as the prefix instruction part of the prompt template. The performance of this model is high variance with the chosen examples vary. Therefore, this template is not taken into account in this section.}
% \footnotetext[9]{The performance of random is obtained by averaging the performance of 5 runs}



% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{sections/Figures/ChatGPT_performance.pdf}
%     \vspace{-0.3in}
%     \caption{The performance comparison of various input prompt templates for ChatGPT. ``Prag.Cause'' stand for \textit{Pragmatic cause} second level sense.   
%     }
%     \label{fig:ChatGPT_performance_figure}
%     \vspace{-0.5cm}
% \end{figure}


==> sections/experiments_setting.tex <==
\section{Experimental Setting}
% In this section, we introduce the details of experimental settings. 

\subsection{Dataset}
The experiments \xin{are} conducted on two datasets, the PDTB 2.0
% \footnote{The License of PDTB 2.0 dataset is LDC User Agreement for Non-Members, and this paper is consistent with their intended use. This dataset download from~\url{https://catalog.ldc.upenn.edu/LDC2008T05}}
~\cite{DBLP:conf/lrec/PrasadDLMRJW08} and the CoNLL-2016 shared task
% \footnote{ CoNLL16 dataset download from~\url{https://www.cs.brandeis.edu/~clp/conll16st/dataset.html}.}
~\cite{DBLP:conf/conll/XueNPRWWW16}, to validate the performance of our method.
% The PDTB 2.0 is a large-scale corpus containing 2,312 Wall Street Journal (WSJ) articles, which includes three sense levels (i.e., classes, types, and sub-types). In this dataset, we validate our model on two popular settings of the PDTB 2.0 dataset, which are the Ji-setting~\cite{DBLP:journals/tacl/JiE15} and Lin-setting~\cite{DBLP:conf/emnlp/LinKN09}. The CoNLL-2016 shared task provides more abundant annotation (e.g., second-level sense type) for shadow discourse parsing. This task includes two test sets, the PDTB section 23 (CoNLL-Test) and newswire texts (CoNLL-Blind), that comply with the PDTB annotation guidelines. We mainly evaluate our model on the top-level and second-level implicit discourse relation by the previous studies~\cite{DBLP:conf/aaai/WuCGLZS22, conf/emnlp/Contrastive_Learning,DBLP:journals/corr/abs-2210-07032} in these datasets. More specific details of the dataset and data statistics are in Appendix~\ref{sec:appendix_data_statistics}.
\xin{
Both contain the Wall Street Journal (WSJ) articles, the difference is the annotation and relation senses.
We evaluate performance on PDTB 2.0 according to two different settings denoted as \textit{Ji}~\cite{DBLP:journals/tacl/JiE15} and \textit{Lin}~\cite{DBLP:conf/emnlp/LinKN09} with 11 subtypes.
The CoNLL-2016 shared task provides more abundant annotations and two test data denoted as \textit{Test} and \textit{Blind} with 15 subtypes.
More specific details and statistics are listed in Appendix~\ref{sec:appendix_data_statistics}.
}



% The former one following~\citet{DBLP:journals/tacl/JiE15, DBLP:conf/ijcai/LiuOSJ20} to split sections 2-20, 0-1, and 21-22 as training, validation, and test sets respectively, while the latter follows ~\citet{DBLP:conf/emnlp/LinKN09, DBLP:conf/acl/HeWGH20} split sections 2-21, 22, 23 as training, validation, and test sets respectively. We evaluate our model on the four top-level implicit discourse senses and the 11 major second-level implicit discourse senses~\cite{DBLP:conf/aaai/WuCGLZS22, conf/emnlp/Contrastive_Learning,DBLP:journals/corr/abs-2210-07032}. The data statistics of the top-level and second-level senses are displayed in Table~\ref{table:pdtb_statistics} and Table~\ref{table:pdtb_Sec_level_statistics} in the Appendix~\ref{sec:appendix_data_statistics}.

% which lexically-grounded annotated discourse relations and the argument structure of discourse relations.
% For the top level, which most work foucused on, including \textit{Comparison} (\textit{Comp.}), \textit{Contingency} (\textit{Cont.}), \textit{Expansion} (\textit{Exp.}), and \textit{Temporal} (\textit{Temp.}). Table~\ref{table:pdtb_statistics} shows the statistics of the top-level senses.

% \paragraph{The CoNLL-2016 Shared Task (CoNLL16)}
% The CoNLL-2016 shared task\footnote{ CoNLL16 dataset download from~\url{https://www.cs.brandeis.edu/~clp/conll16st/dataset.html}.}~\cite{DBLP:conf/conll/XueNPRWWW16} provides more abundant annotation (e.g., second-level sense type) for shadow discourse parsing. This task includes two test sets, the PDTB section 23 (CoNLL-Test) and newswire texts (CoNLL-Blind), that comply with the PDTB annotation guidelines. Compared with PDTB 2.0, CoNLL16 includes more new class sense (e.g., \textit{Contingency.Condition}) and merges several labels to annotate new labels. For example, \textit{Contingency.Pragmatic cause} is
% merged into \textit{Contingency.Cause.Reason} to remove the former type with very few samples. In this paper, we follow~\cite{DBLP:conf/conll/WangL16, Lan2017Multi, DBLP:conf/ijcai/LiuOSJ20} to perform the experiments on this CoNLL-2016 dataset and validate the performance of our model in the top- and second-level sense.    


\subsection{Implementation Details}
% We employ the T5 model~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} as our backbone model and primarily use T5-large to compare with extensive baselines. We utilized the \textit{T5ForConditionalGeneration} to acquire the prediction score over each label word at each <mask> token position. Generally, the overall configuration follows the setting in \citet{DBLP:conf/emnlp/LesterAC21} and sets the learnable prompt length as 20. The training is implemented using cross-entropy loss with the training steps are 30,000. We adopt an Adafactor optimizer~\cite{DBLP:conf/icml/ShazeerS18} and select various learning rate ranges for different dataset settings, which yields the best performance on the validation set. The specific hyperparameters are listed in Table~\ref{table:Implementation_details_hypreparameters}. The batch size and maximum input sequence are 4 and 350. The maximum generates sequence length of the encoder is 10. Accuracy and Macro F1 score are used as the evaluation metric for all experiments in this task\footnote{Some data instances in PDTB and CoNLL were annotated with multiple labels. Following the previous study and the scorer at \url{https://github.com/attapol/conll16st}, a prediction is considered correct whenever it matches one of the ground-truth labels.}. We select the best model that
% yields the best performance on the validation set. Our model is conducted on two 32GB NVIDIA V100 GPUs, except for the T5-11b scale on two 48GB NVIDIA A6000 GPUs. The running time for T5-base is around 8 hours, while T5-large is around 19 hours. Since we are interested in the ability of our method with adopt a larger-scale model on this task, we tested the T5-11b model on various settings. Most of the configuration is the same as the above T5-large version. Some slight differences are batch size is one, gradient accumulation step is 16, and the running time is around 50 hours. 

% The T5 model~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}\footnote{The frozen \jy{pre-trained} T5 model download from Hugging Face~\url{https://huggingface.co/}.} is employed as our backbone model and primarily uses T5-large to compare with extensive baselines. We utilized the \textit{T5ForConditionalGeneration} to acquire the prediction score over each label word at each <mask> token position. Generally, the overall the configuration follows the setting in \citet{DBLP:conf/emnlp/LesterAC21} and we showed more details of the configuration in Appendix~\ref{sec:appendix_discoPrompt_implementation_details}. Accuracy and Macro F1 score are used as the evaluation metric for all experiments in this task\footnote{Some data instances in PDTB2.0 and CoNLL2016 were annotated with multiple labels. Following the previous study and the scorer at \url{https://github.com/attapol/conll16st}, a prediction is considered correct whenever it matches one of the ground-truth labels.}.
\xin{
We employ the T5 model~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} as the backbone to implement \textbf{DiscoPrompt} and use the T5-large as the primary model for a fair comparison with extensive baselines.
Generally, the overall configuration follows the setting in \citet{DBLP:conf/emnlp/LesterAC21}, and we put more details of the configuration in Appendix~\ref{sec:appendix_discoPrompt_implementation_details}.
We report the Macro-F1 score and accuracy in experiments and ablation studies.
A prediction is considered as correct whenever it matches one of the ground-truth labels.
All experiments are conducted with 2 $\times$ NVIDIA V100 (32\text{GB}) except for the T5-11b scale on  2 $\times$ NVIDIA A6000 (48\text{GB}). 
}

\subsection{Baselines}
This paper mainly adopts two categories of competitive baselines for the PDTB 2.0 dataset and the CoNLL-2016 task\footnote{We report our produced results via the official code if the authors did not report results on those data.}. The first category is the previous \jy{state-of-the-art} (SOTA) baselines, such as TransS\cite{DBLP:conf/acl/HeWGH20}, BMGF-RoBERTa~\cite{DBLP:conf/ijcai/LiuOSJ20}, LDSGM~\cite{DBLP:conf/aaai/WuCGLZS22}, XLNet-large~\cite{DBLP:conf/acl/KimFGL20}, OTMT (XLNet-large)~\cite{DBLP:conf/www/JiangQL22}, and ContrastiveIDRR~\cite{conf/emnlp/Contrastive_Learning}.
Two partitions of these SOTA baselines are highlighted for comparison with our method.
One partition utilizes the hierarchical information in their methods (e.g., the LDSGM and ContrastiveIDRR), and \xin{the other is to fine-tune} the \jy{pre-trained} language models (e.g., XLNet-large). \xin{Therefore, we include the fine-tuned T5 models to illustrate the performance gain of prompt tuning.} \xin{Besides, a prompt-based method PCP~\cite{DBLP:journals/corr/abs-2210-07032} and general Prefix-Tuning~\cite{DBLP:conf/acl/LiL20} as well as Prompt Tuning~\cite{DBLP:conf/emnlp/LesterAC21} are included.}The details of implementation \jy{are} listed in~\ref{sec:Appendix_baseline_mdoels}.




% and ~\ref{sec:implement_details_prompt_baseline}.
% Moreover, we include the fine-tuning T5 model in the latter partition to show the improvement of our method against the fine-tuning T5 model.
% Another category is the prompt-based methods, such as PCP~\cite{DBLP:journals/corr/abs-2210-07032}, Prompt Tuning~\cite{DBLP:conf/emnlp/LesterAC21}, and Prefix-Tuning~\cite{DBLP:conf/acl/LiL20}.

% The implementation details of the Prompt Tuning and Prefix-Tuning methods are appended in Appendix~\ref{sec:implement_details_prompt_baseline}.
% Apart from the baselines mentioned above, we include the extensive previous state-of-the-air baselines in Table~\ref{tab:Appendix_discourserelation_classification_pdtb2.0} in Appendix.
% More details of the baseline are in Appendix~\ref{sec:Appendix_baseline_mdoels}.

